Enabling Work-conserving Bandwidth Guarantees for Multi-tenant Datacenters via Dynamic Tenant-Queue Binding

Today's cloud networks are shared among many tenants. Bandwidth guarantees and work conservation are two key properties to ensure predictable performance for tenant applications and high network utilization for providers. Despite significant efforts, very little prior work can really achieve both properties simultaneously even some of them claimed so. In this paper, we present QShare, an in-network based solution to achieve bandwidth guarantees and work conservation simultaneously. QShare leverages weighted fair queuing on commodity switches to slice network bandwidth for tenants, and solves the challenge of queue scarcity through balanced tenant placement and dynamic tenant-queue binding. QShare is readily implementable with existing switching chips. We have implemented a QShare prototype and evaluated it via both testbed experiments and simulations. Our results show that QShare ensures bandwidth guarantees while driving network utilization to over 91% even under unpredictable traffic demands.

==> background.tex <==
\section{BACKGROUND}
Several well-known models (\eg the hose model~\cite{hose, oktopus, faircloud, elasticswitch}, 
Pipe model~\cite{secondnet} and TAG~\cite{tag}) have been proposed to 
formulate tenant bandwidth guarantees. 
Then guided by a VM placement algorithm, network operators embed tenants 
into data centers. The algorithm ensures that the embedded tenants' bandwidth guarantees are accomplished whereas 
tenants whose bandwidth guarantees cannot be satisfied are rejected. 
Regardless of which model is adopted, network operators have to relay 
on rate limiters on hypervisors to enforce bandwidth guarantees. 


Merely relaying on endhost rate limiters has the following shortcomings and limitations. 
To begin with, the expense of running large number of rate limiters on hypervisors 
is non-trivial. For instance, in ElasticSwitch~\cite{elasticswitch}, assume one tenant 
has $15$ VMs on one hypervisor and another $15$ VMs on another hypervisor and 
they have the many-to-many communication pattern. Then each hypervisor 
has to keep $2{\times}15{\times}15{=}450$ rate limiters for a single tenant (including both 
inbound and outbound bandwidth guarantees). As 
one hypervisor can host VMs for multiple tenants, it needs to run considerable 
amount of rate limiters in real deployment. 

More importantly, using rate limiters to enforce bandwidth guarantees potentially 
makes it more difficult to achieve work conservation. Specifically, 
when some VMs do not fully consume their guarantees, other VMs cannot 
boot their rates to use the available bandwidth since their rates are 
determined by their rate limiters, which are computed without realizing 
real traffic demands. Therefore, ElasticSwitch~\cite{elasticswitch} proposes 
a rate allocation (RA) process to assign the unused bandwidth among 
tenants to achieve work conservation. However, such a complete 
end-to-end solution may not work well in data center context. To begin with, 
RA estimate the available bandwidth based on the network congestion over 
a period of time ($15$ms in their implementation). However, given the highly bursty
traffic load in data centers, flows may have already finished before RA assigns 
the spare bandwidth. Also, malicious tenants can synchronize their traffic 
to deliberately cause congestion and fake a congested network 
so as to stop other tenants increasing their rates. 
Furthermore, treating data center network as a blackbox creates 
an inevitable trade-off between achieving bandwidth guarantees and being 
work-conversing. This is because work-conservation requires RA 
to aggressively assign leftover bandwidth which may violate bandwidth guarantees 
given that the estimation of unused bandwidth is never accurate. 
